Lingshu-Cell: A generative cellular world model for transcriptome modeling toward virtual cells

Modeling cellular states and predicting their responses to perturbations are central challenges in computational biology and the development of virtual cells. Existing foundation models for single-cell transcriptomics provide powerful static representations, but they do not explicitly model the distribution of cellular states for generative simulation. Here, we introduce Lingshu-Cell, a masked discrete diffusion model that learns transcriptomic state distributions and supports conditional simulation under perturbation. By operating directly in a discrete token space that is compatible with the sparse, non-sequential nature of single-cell transcriptomic data, Lingshu-Cell captures complex transcriptome-wide expression dependencies across approximately 18,000 genes without relying on prior gene selection, such as filtering by high variability or ranking by expression level. Across diverse tissues and species, Lingshu-Cell accurately reproduces transcriptomic distributions, marker-gene expression patterns and cell-subtype proportions, demonstrating its ability to capture complex cellular heterogeneity. Moreover, by jointly embedding cell type or donor identity with perturbation, Lingshu-Cell can predict whole-transcriptome expression changes for novel combinations of identity and perturbation. It achieves leading performance on the Virtual Cell Challenge H1 genetic perturbation benchmark and in predicting cytokine-induced responses in human PBMCs. Together, these results establish Lingshu-Cell as a flexible cellular world model for in silico simulation of cell states and perturbation responses, laying the foundation for a new paradigm in biological discovery and perturbation screening.

==> sections/backmatter.tex <==
\backmatter





\section*{Declarations}

\begin{itemize}
\item Data availability 

All datasets used in this study are publicly available. The PARSE 10M PBMC dataset, used for both unconditional generation and cytokine perturbation experiments, is available at \url{https://parse-wget.s3.us-west-2.amazonaws.com/10m/10M_PBMC_12donor_90cytokines_h5ad_20260203.zip}. Human, mouse, and rhesus macaque data were accessed through the CZ CELLxGENE Census API (\url{https://chanzuckerberg.github.io/cellxgene-census/index.html}; census version: 2025-11-08). Zebrafish and fly sample metadata were obtained from the scBaseCount public release hosted on Google Cloud Storage at \texttt{gs://arc-ctc-scBaseCount/2025-02-25}, using the species-specific \texttt{sample\_metadata.parquet} files from the \texttt{GeneFull\_Ex50pAS} collection. The Virtual Cell Challenge H1 dataset was obtained from the public release hosted on Google Cloud Storage at \texttt{gs://arc-institute-virtual-cell-atlas/virtual-cell-challenge/}. Additional genetic perturbation datasets from Replogle et al., Nadig et al., Jiang et al., and X-Atlas/Orion are available at \url{https://doi.org/10.25452/figshare.plus.20029387
        
        }, \url{https://www.ncbi.nlm.nih.gov/geo/query/acc.cgi?acc=GSE264667}, \url{https://zenodo.org/records/14518762}, and \url{https://doi.org/10.25452/figshare.plus.29190726
        
        }, respectively. The datasets analyzed in this study were defined according to the filtering procedure described in Appendix A.

\end{itemize}

